Graceful Degradation of Air Traffic Operations

The introduction of new technologies and concepts of operation in the air transportation system is not possible, unless they can be proven not to adversely affect the system operation under not only nominal, but also degraded conditions. In extreme scenarios, degraded operations due to partial or complete technological failures should never endanger system safety. Many past system evolutions, whether ground-based or airborne, have been based on trial-and-error, and system safety was addressed only after a specific event yielded dramatic or near- dramatic consequences. Future system evolutions, however, must leverage available computation, prior knowledge and abstract reasoning to anticipate all possible system degradations and prove that such degradations are graceful and safe. This paper is concerned with the graceful degradation of high-density, structured arrival traffic against partial or complete surveillance failures. It is shown that for equal performance requirements, some traffic configurations might be easier to handle than others, thereby offering a quantitative perspective on these traffic configurations. ability to "gracefully degrade". To support our work, we also introduce a new conflict resolution algorithm, aimed at solving conflicts involving many aircraft when aircraft position information is in the process of degrading.

==> sameSpeed.tex <==
\subsection{Identical speeds case}
For the sake of computing simplicity, we assume all aircraft share the same speed $V$. This assumption simplifies the formulae for $\theta_{ij}$ and $\alpha_{ij}$ and allows us to obtain piecewise linear approximations. 

\subsubsection{Expression of the angle of the relative velocity: $\theta_{ij}$}
Using the assumption of identical speed, the angle between the relative velocity and the $x$-axis, the expression of $\theta_{ij}$ given by equation \ref{eq:thetaij} can be simplified : 
\begin{equation}
\begin{split}
\theta_{ij} &= \arctan\frac{\sin\theta_i - \sin\theta_j}{\cos\theta_i - \cos\theta_j}\\
&=\arctan\frac{\sin(\frac{\theta_i{-}\theta_j}{2})\cos(\frac{\theta_i{+}\theta_j}{2})}{-\sin(\frac{\theta_i{-} \theta_j}{2})\sin(\frac{\theta_i{+}\theta_j}{2})}.\\
\end{split}
\label{eq:thetaijLinear}
\end{equation}
$\theta_{ij}$ is a function of $\theta_i + \theta_j$ and $\theta_i - \theta_j$.  It can be shown that $\theta_{ij}$ is a piecewise affine function of $\theta_i + \theta_j$ and $\theta_i - \theta_j$ of the form $\theta_{ij} = m_{ij} (\theta_i + \theta_j) + p_{ij}$. The value of $m_{ij}$ if always $\tfrac{1}{2}$ and the values taken by $p_{ij}$  are summarized in table \ref{tab:ThetaijmCoef}.

\renewcommand{\arraystretch}{1.5}
\begin{table}[ht]
\begin{center}
    \begin{tabular}{|p{0.1\linewidth}|p{0.1\linewidth}|p{0.20\linewidth}|}
    \hline
    \multicolumn{1}{|c|}{Case 1}
    &\multicolumn{1}{|c|}{$\theta_i - \theta_j < 0$ and $-2\pi \leq \theta_i + \theta_j < -\pi$}
    &\multicolumn{1}{|l|}{$p_{ij} = \frac{3\pi}{2}$}\\
    \hline
    \multicolumn{1}{|c|}{Case 2}
    &\multicolumn{1}{|c|}{$\theta_i - \theta_j < 0$ and $-\pi \leq \theta_i + \theta_j < 2\pi$}
    &\multicolumn{1}{|l|}{$p_{ij} = -\frac{\pi}{2}$}\\
    \hline
    \multicolumn{1}{|c|}{Case 3}
    &\multicolumn{1}{|c|}{$\theta_i - \theta_j \geq 0$ and $-2\pi \leq \theta_i + \theta_j < \pi$}
    &\multicolumn{1}{|l|}{$p_{ij} = \frac{\pi}{2}$}\\
    \hline
    \multicolumn{1}{|c|}{Case 4}
    &\multicolumn{1}{|c|}{$\theta_i - \theta_j \geq 0$ and $\pi \leq \theta_i + \theta_j < 2\pi$}
    &\multicolumn{1}{|l|}{$p_{ij} = -\frac{3\pi}{2}$}\\
    \hline
    \end{tabular}\caption{Intercept coefficient of $\theta_{ij}$}\label{tab:ThetaijmCoef}
\end{center}
\end{table}

% Table \ref{tab:Thetaij} presents the expression of $\theta_{ij}$ function of $\theta_i + \theta_j$ and $\theta_i - \theta_j$.


% \renewcommand{\arraystretch}{1.5}
% \begin{table}
% \begin{center}
%     \begin{tabular}{|p{0.13\linewidth}|p{0.20\linewidth}|p{0.20\linewidth}|p{0.20\linewidth}|p{0.2\linewidth}|p{0.20\linewidth}|}
%     \hline
%     &\multicolumn{1}{|c|}{$-2\pi \leq \theta_i + \theta_j < -\pi$}
%     &\multicolumn{1}{|c|}{$-\pi \leq \theta_i + \theta_j < 0$}
%     &\multicolumn{1}{|c|}{$0 \leq \theta_i + \theta_j < \pi$}
%     &\multicolumn{1}{|c|}{$\pi \leq \theta_i + \theta_j < 2\pi$}\\
%     \hline
%     \multicolumn{1}{|c|}{$\theta_i - \theta_j < 0$}
%     &\multicolumn{1}{|c|}{$\theta_{ij} = \frac{\theta_i + \theta_j}{2}+\frac{3\pi}{2}$}
%     &\multicolumn{1}{|c|}{$\theta_{ij} = \frac{\theta_i + \theta_j}{2}-\frac{\pi}{2}$}
%     &\multicolumn{1}{|c|}{$\theta_{ij} = \frac{\theta_i + \theta_j}{2}-\frac{\pi}{2}$}
%     &\multicolumn{1}{|c|}{$\theta_{ij} = \frac{\theta_i + \theta_j}{2}-\frac{\pi}{2}$}\\
%     \hline
%     \multicolumn{1}{|c|}{$0 \leq \theta_i - \theta_j$}
%     &\multicolumn{1}{|c|}{$\theta_{ij} = \frac{\theta_i + \theta_j}{2}+\frac{\pi}{2}$}
%     &\multicolumn{1}{|c|}{$\theta_{ij} = \frac{\theta_i + \theta_j}{2}+\frac{\pi}{2}$}
%     &\multicolumn{1}{|c|}{$\theta_{ij} = \frac{\theta_i + \theta_j}{2}+\frac{\pi}{2}$}
%     &\multicolumn{1}{|c|}{$\theta_{ij} = \frac{\theta_i + \theta_j}{2}-\frac{3\pi}{2}$}\\
%     \hline
%     \end{tabular}\label{tab:Thetaij}\caption{$\theta_{ij}$ function of $\theta_i + \theta_j$ and $\theta_i - \theta_j$}
% \end{center}
%\end{table*}




% \begin{table}[ht]
% \begin{center}
%     \begin{tabular}{|p{0.13\linewidth}|p{0.20\linewidth}|p{0.20\linewidth}|p{0.20\linewidth}|p{0.2\linewidth}|p{0.20\linewidth}|}
%     \hline
% 	&\multicolumn{1}{|c|}{$\theta_i - \theta_j < 0$}
% 	& \multicolumn{1}{|c|}{$0 \leq \theta_i - \theta_j$}\\
% 	\hline
% 	 \multicolumn{1}{|c|}{$-2\pi{\leq}\theta_i{+}\theta_j{<}-\pi$} 
% 	&\multicolumn{1}{|c|}{$\theta_{ij}{=}\frac{\theta_i + \theta_j}{2}+\frac{3\pi}{2}$}
% 	&\multicolumn{1}{|c|}{$\theta_{ij}{=}\frac{\theta_i + \theta_j}{2}+\frac{\pi}{2}$}\\ [1ex]
% 	\hline
%     	\multicolumn{1}{|c|}{$-\pi{\leq}\theta_i{+}\theta_j{<}0$}
% 	&\multicolumn{1}{|c|}{$\theta_{ij}{=}\frac{\theta_i + \theta_j}{2}-\frac{\pi}{2}$}   
% 	&\multicolumn{1}{|c|}{$\theta_{ij}{=}\frac{\theta_i + \theta_j}{2}+\frac{\pi}{2}$}\\ [1ex]
% 	\hline
%  	\multicolumn{1}{|c|}{$0{\leq}\theta_i{+}\theta_j{<}\pi$}
% 	&\multicolumn{1}{|c|}{$\theta_{ij}{=}\frac{\theta_i + \theta_j}{2}-\frac{\pi}{2}$}
% 	&\multicolumn{1}{|c|}{$\theta_{ij}{=}\frac{\theta_i + \theta_j}{2}+\frac{\pi}{2}$}\\ [1ex]
% 	\hline
% 	\multicolumn{1}{|c|}{$\pi{\leq}\theta_i{+}\theta_j{<}2\pi$}
%  	&\multicolumn{1}{|c|}{$\theta_{ij}{=}\frac{\theta_i + \theta_j}{2}-\frac{\pi}{2}$}
%  	&\multicolumn{1}{|c|}{$\theta_{ij}{=}\frac{\theta_i + \theta_j}{2}-\frac{3\pi}{2}$}\\ [1ex]
%     \hline
%     \end{tabular}\caption{$\theta_{ij}$ function of $\theta_i + \theta_j$ and $\theta_i - \theta_j$}\label{tab:Thetaij}
% \end{center}
% \end{table}

% \begin{figure}[ht]
% \centering
%     \includegraphics*[scale=0.3, viewport = 0 50 720 720]{pics/thetaij.pdf}
%     \caption{$\theta_{ij}$ function of $\theta_i + \theta_j$ and $\theta_i - \theta_j$}
% \label{fig:thetaij}
% \end{figure}
We can determine the value of $p_{ij}$ using boolean variables. Let $bCaseDiffPos_{ij}$, $ bCaseSumInfmPi_{ij}$, $bCaseSumSupPi_{ij}$, $bCase1_{ij}$ and $bCase4_{ij}$ be boolean variables such that:
\begin{align}
&bCaseDiffPos_{ij} =1 \Longleftrightarrow \theta_i - \theta_j \geq 0\\
&bCaseSumInfmPi_{ij} = 1 \Longleftrightarrow  -2\pi \leq \theta_i + \theta_j < -\pi\\
&bCaseSumSupPi_{ij} = 1 \Longleftrightarrow \pi \leq \theta_i + \theta_j < 2\pi\\
&bCase1_{ij}=1 \Longleftrightarrow
\begin{cases}
&bCaseDiffPos_{ij} = 0\\
&\text{and} \\
&bCaseSumInfmPi_{ij} = 1
\end{cases}\\
&bCase4_{ij}=1 \Longleftrightarrow
\begin{cases}
&bCaseDiffPos_{ij} = 1\\
&\text{and} \\
&bCaseSumSupPi_{ij} = 1\\
\end{cases}\\
\end{align}

Those 3 boolean variables yield the following expression for $p_{ij}$ and hence $\theta_{ij}$:
\begin{equation}
p_{ij}{=}(bCaseSumPos_{ij}-\tfrac{1}{2})\pi + 2\pi(bCase1_{ij} - bCase4_{ij}),\\
\end{equation}
\begin{multline}
 \theta_{ij} = \frac{\theta_i + \theta_j}{2} + (bCaseDiffPos_{ij}-\tfrac{1}{2})\pi + \ldots\\ 
\hspace{2cm} 2\pi(bCase1_{ij} - bCase4_{ij}),
\end{multline}
which is linear in $\theta_i$ and $\theta_j$ and in the boolean variables.





\subsubsection{Constraints formulation for $\theta_{ij}$}
The following formulation uses the big-$M$ method. $M$ is a large number such that if multiplied by a boolean set to 1, the constraint is always satisfied, whatever the value of the other variables. This enables us to select between constraints and use $or$ relationship between constraints. This is a standard procedure described  \cite{OperationsResearch}.
 
Determination of the sign of  $\theta_i - \theta_j$:
\begin{multline}
bCaseDiffPos_{ij} = 1 \Longleftrightarrow\\
\begin{cases}
\theta_i - \theta_j  - M bCaseDiffPos_{ij} < 0,\\
-\theta_i + \theta_j - M (1-bCaseDiffPos_{ij}) < 0.
\end{cases}\\
\end{multline}
Determination of the boolean $bCaseSumInfmPi_{ij}$ if $\theta_i + \theta_j < -\pi$:
\begin{multline}
bCaseSumInfmPi_{ij} = 1 \Longleftrightarrow\\
\begin{cases}
\theta_i + \theta_j + \pi - M (1-bCaseSumInfmPi_{ij}) < 0,\\
-\theta_i - \theta_j - \pi - M bCaseSumInfmPi_{ij} < 0.
\end{cases}\\
\end{multline}
Determination if $\theta_i + \theta_j \geq \pi$:
\begin{multline}
bCaseSumInfmPi_{ij} = 1 \Longleftrightarrow\\
\begin{cases}
-\theta_i - \theta_j + \pi - M (1-bCaseSumSupPi_{ij}) \leq 0,\\
\theta_i + \theta_j - \pi - M bCaseSumSupPi_{ij} \leq 0.
\end{cases}\\
\end{multline}
Determination of the boolean $bCase1_{ij}$:
\begin{multline}
bCase1_{ij} = 1 \Longleftrightarrow\\
\begin{cases}
-1.5 + bCaseDiffPos_{ij} - \ldots \\
\quad bCaseSumInfmPi_{ij} + 2bCase1_{ij} \leq 0,\\
-0.5 - 2bCaseDiffPos_{ij}  \ldots\\
 \quad  + bCaseSumInfmPi_{ij} - bCase1_{ij} \leq 0,.
\end{cases}\\
\end{multline}
Determination of the boolean $bCase4_{ij}$:
\begin{multline}
bCase4_{ij} = 1 \Longleftrightarrow\\
\begin{cases}
1.5 - bCaseDiffPos_{ij} - bCaseSumSupPi_{ij} \ldots \\
\quad- 2(1-bCase4_{ij}) \leq 0,\\
 -1.5 + bCaseDiffPos_{ij} + bCaseSumSupPi_{ij} \ldots \\
\quad- bCase4_{ij} \leq 0.
\end{cases}\\
\end{multline}



\subsubsection{Cone angular width $2\alpha_{ij}$ in the relative frame of reference}
This section presents the formulas to determine the cone angular width $2\alpha_{ij}$ when aircraft share an identical speed. The assumption leads to $\dot r_i = \dot r, i=1\ldots n$ and
\begin{equation}
\begin{split}
\alpha_{ij} &= \arcsin\frac{2\dot r}{\sqrt{V^2(\cos\theta_i{-}\cos\theta_j)^2{+}V^2(\sin\theta_i{-}\sin\theta_j)^2}}\\
&= \arcsin\frac{\dot r}{V|\sin(\frac{\theta_i-\theta_j}{2})|}\\
&= \arcsin\frac{\tan\Delta\theta}{|\sin(\frac{\theta_i-\theta_j}{2})|}
\end{split}
\label{eq:alpha}
\end{equation}


The half cone angular width $\alpha_{ij}$ is given by equation (\ref{eq:alpha}) and it is a non linear function of $\theta_i - \theta_j$.  This function is symmetric about $\theta_i - \theta_j = 0$ and consists of two quasi convex components, separated at $\theta_i - \theta_j = 0$, as shown in Figure \ref{fig:alphaLinear}. The epigraph of each of these quasi convex components can be approximated by the intersection of linear constraints defined by their
slopes $a_k$ and intercepts $b_k$. Using the big-$M$ method allows us to account for the presence of two disconnected components, and this linearization leads to:

\begin{figure}[ht]
\centering
    \includegraphics*[scale=0.40,viewport=75 0 700 315 ]{alphaLineair.png}
    \caption{$\alpha_{ij}$ function of $\theta_i-\theta_j$ and the linearization used}
\label{fig:alphaLinear}
\end{figure}


\begin{equation}
\begin{split}
&a_1(\theta_i-\theta_j) + b_1 - M bCaseAlphaPos_{ij} \leq \alpha_{ij}\\
&a_2(\theta_i-\theta_j) + b_2 - M bCaseAlphaPos_{ij} \leq \alpha_{ij}\\
\vdots\\
&a_l(\theta_i-\theta_j) + b_l - M bCaseAlphaPos_{ij} \leq \alpha_{ij}\\
&-a_1(\theta_i-\theta_j) + b_1 - M(1 - bCaseAlphaPos_{ij}) \leq \alpha_{ij}\\
&-a_2(\theta_i-\theta_j) + b_2 - M(1 - bCaseAlphaPos_{ij}) \leq \alpha_{ij}\\
\vdots\\
&-a_l(\theta_i-\theta_j) + b_l - M(1 - bCaseAlphaPos_{ij}) \leq \alpha_{ij}
\end{split}
\end{equation}
with $bCaseAlphaPos_{ij}$ a binary variable used to transform the $or$ between the constraints in an $and$ relationship.

The avoidance constraints are now given by:
\begin{align}
\begin{cases}\label{eq:avoidanceConstraints}
    -\frac{\theta_i + \theta_j}{2} - (\frac{1}{2} - bCasePlus_{ij})\pi + \omega_{ij} + \alpha_{ij} \ldots\\
\quad + \hat\gamma_{ij} - M bCaseIneqPos_{ij} < 0\\
\text{and} \\
    \frac{\theta_i + \theta_j}{2} + (\frac{1}{2} - bCasePlus_{ij})\pi - \omega_{ij} + \alpha_{ij}  \ldots\\
\quad + \hat\gamma_{ij} - M(1 - bCaseIneqPos_{ij}) <0
\end{cases}
\end{align}
with $bCaseIneqPos_{ij}$ a binary variable used to transform the $or$ between the constraints in an $and$ relationship.




\subsubsection{Mixed constraints for conflict avoidance}
The conflict avoidance constraints given by equation \ref{eq:generalAvoidanceConstraints} can be handled in a linear programming framework by using the big-$M$ method, leading to the following mixed constraints: 

\begin{align}
\begin{cases}
    -\frac{\theta_i + \theta_j}{2} - (\frac{1}{2} - bCasePlus_{ij})\pi + \omega_{ij} + \tilde\gamma_{ijr_0} \ldots\\
\quad - M bCaseIneqPos_{ij} - M b1_{ij} < 0\\
    \frac{\theta_i + \theta_j}{2} + (\frac{1}{2} - bCasePlus_{ij})\pi - \omega_{ij} + \tilde\gamma_{ijr_0} \ldots\\ 
\quad - M(1 - bCaseIneqPos_{ij}) - M b1_{ij} <0\\
    -\frac{\theta_i + \theta_j}{2} - (\frac{1}{2} - bCasePlus_{ij})\pi + \omega_{ij} + \alpha_{ij} + \hat\gamma_{ijr_f} \ldots\\ \quad-  M bCaseIneqPos_{ij} - M b2_{ij} < 0\\
    \frac{\theta_i + \theta_j}{2} + (\frac{1}{2} - bCasePlus_{ij})\pi - \omega_{ij} + \alpha_{ij} + \hat\gamma_{ijr_f} \ldots\\ \quad- M(1 - bCaseIneqPos_{ij}) - M b2_{ij} <0\\
   -\frac{\theta_i + \theta_j}{2} - (\frac{1}{2} - bCasePlus_{ij})\pi + \omega_{ij} + \frac{\alpha_{ij}}{2} + \gamma^\ast_{ijr_f} \ldots\\ 
\quad- M bCaseIneqPos_{ij} - M b3_{ij}< 0\\
    \frac{\theta_i + \theta_j}{2} + (\frac{1}{2} - bCasePlus_{ij})\pi - \omega_{ij} + \frac{\alpha_{ij}}{2} + \gamma^\ast_{ijr_f}\ldots\\ \quad - M(1 - bCaseIneqPos_{ij}) - M b3_{ij} <0\\
b1_{ij} + b2_{ij} + b3_{ij} = 2\\
\end{cases}
\end{align}
with $b1_{ij}, b2_{ij}$ and $b3_{ij}$ binary variables. 

The global algorithm consists on minimizing expression \ref{eq:min} subject to all the constraints previously developed. We wrote the constraints in an AMPL format and solved using CPLEX. MATLAB was used to generate the 1650 cases and was also used for the post-processing. The computing time to solve an 8 aircraft configuration ranged from less than a second to dozen of seconds on a 4-processor, Pentium  class computer. 


% The algorithm previously developed (GRAA) considers an uncertainty with growing radius unlimited in time. This is very conservative and restricts the algorithm to a limited number of aircraft: the radius of avoidance infinitely grow, hence, will tend to cover all the airspace. This is not realistic considering that there will almost always be another positioning system. This later one will certainly be less accurate. Hence, we now consider a growing radius of avoidance, but the growth is limited in time: Once the radius reached a given size, it stops growing. This can model the transition from a very accurate positioning system such as ADS-B to a less accurate one, such as Primary Surveillance Radar.
% 
% Let denote by $r_i$ the initial radius of avoidance, $r_f$ the final radius of avoidance and $\dot r$ the growing rate.
% The avoidance process is now divided in two parts:
% \begin{itemize}
% \item The conflict will occur while the circle of avoidance is growing.
% \item The conflict will occur after the circle of avoidance reached its maximum $r_f$.
% \end{itemize}
% In the first case the GRAA is used, and in the second case, an avoidance algorithm (AA) such as presented in \cite{PallottinoConflitResolution} is used. The radius of avoidance is set at $r_f$. This AA is the GRAA setting $\alpha_{ij} = 0$ and $r = r_f$.
% 
% The main issue is to determine when each algorithm should be used, as it depends on the initial distance between the aircraft and the relative velocity after the change of heading. As the relative velocity after the heading change is unknown, we can not, a-priori choose which algorithm to use. We let CPLEX do it by adding 2 avoidance constraints corresponding to the AA with radius of avoidance $r_f$. A ``or'' boolean variable $bAA$ is introduced to choose between the AA and GRAA ($bAA = 1$ if the AA is used, $0$ otherwise). Then, avoidance constraints (\ref{eq:avoidanceConstraints}) are replaced by:
% 

% 
% If $2r_f  > D_{ij} $, we set  $\gamma_{ijr_f}$ at $2\pi$ so that the AA can not be used. 






% \subsection{Optimization of the arrival process}
% If a degradation happens around an airport an particularly affects the arrival process, the previous algorithm is not optimal: all the aircraft are safely spread out but only one can land. Reducing the number of aircraft flying reduces the complexity and minimizes the overall delay.
% 
% To maximize the number of landings, we add to the algorithm a spacing distance constraint. We assume that the aircraft are converging to a way point. After this way point, they are aligned and ready to land. Let $ac_i$ be the further aircraft from the way point and $d$ the distance from the way point to the runway.
% 
% \begin{equation}
% distToWP_i - distToWP_j(1 + \frac{2\dot r}{V}) - 2R - d >0,
% \end{equation}
% 
% $distToWP_i$ is the initial distance of each aircraft to the way point, $R$ is the circle of avoidance initial radius, $\dot r$ is the increase rate of the circle of avoidance and $V$ is the speed of the aircraft.
% This constraint is satisfied if both aircraft are not deviated and go first to the way point and then to the runway, and their circle of avoidance do not intersect each other before landing.
% 
% To be enabled, this constraint requires both aircraft not to be deviated. The boolean variable $bNoChangeThetaCombination_{ij}$ is set to 1 if and only if none of aircraft $i$ and $j$ is deviated from its initial trajectory. This is done with the following set of constraints.
% 
% \begin{align}
% \begin{cases}
%     1.5 &- bThetaNoChange_i - bThetaNoChange_j \\
%                               &- M*(1-bNoChangeThetaCombination_{ij} \leq0\\
%     -1.5 &+ bThetaNoChange_i + bThetaNoChange_j \\
%                             &- M*bNoChangeThetaCombination_{ij} \leq 0,
% \end{cases}\\
% \end{align}
% 
% where $bThetaNoChange_i$ is a boolean variable set to 1 if aircraft $i$ is not deviated from its initial trajectory.








